GenSpan: Generation-Calibrated Motion Span Priors for Multi-Verb Video Corpus Moment Retrieval

Video Corpus Moment Retrieval (VCMR) aims to retrieve both the correct video and its temporal segment corresponding to a natural-language query, a task that is especially challenging for multi-verb queries where temporal action ordering is critical. Existing approaches often rely solely on text or static images and struggle to capture implicit motion dynamics, leading to retrieval errors and temporal misalignment. We propose GenSpan, a generation-calibrated VCMR framework that constructs short auxiliary videos from LLM-selected subtitle cues and decomposed sub-events, using these as temporal priors rather than direct retrieval targets. A token selector filters candidate-video features aligned with generated motion, and a bidirectional state-space model efficiently predicts video-moment tuples. Experiments on TVR and ActivityNet-Captions demonstrate that GenSpan improves corpus-level retrieval and moment localization, particularly for complex multi-action queries, while reducing computational cost compared to state-of-the-art multimodal baselines.

==> checklist.tex <==
\section*{NeurIPS Paper Checklist}

\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}.
    \item[] Justification: The abstract and introduction state that GenSpan uses generated temporal priors and token selection for VCMR, and the experiments report VCMR, VMR, VR, ablations, efficiency, and multi-verb analyses that support these claims.

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{}.
    \item[] Justification: The conclusion and analysis discuss sensitivity to generated-prior quality, including hallucinated or semantically incomplete generated clips, and note future directions such as stronger generators or audio cues.

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{}.
    \item[] Justification: The paper is empirical and does not introduce theoretical results, theorems, or formal proofs.

\item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerNo{}.
    \item[] Justification: The code is not included in the initial submission, but the paper provides detailed implementation and training details. We plan to release the code and processed annotations upon acceptance.

\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerNo{}.
    \item[] Justification: The initial submission does not include a public code release. We use public datasets and plan to release anonymized code and processed annotations after acceptance.

\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer) necessary to understand the results?
    \item[] Answer: \answerYes{}.
    \item[] Justification: The experiments section and appendix specify datasets, splits, metrics, model components, keep ratio, optimizer, learning rate, batch size, epochs, loss weights, generation settings, and inference protocol.

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNo{}.
    \item[] Justification: The paper reports deterministic benchmark metrics and ablations but does not include error bars or statistical significance tests due to the high cost of repeated text-to-video generation and full VCMR training.

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{}.
    \item[] Justification: The paper reports training on NVIDIA RTX 4090 GPUs and includes memory comparisons for Transformer and GenSpan variants under different sequence lengths.

\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{}.
    \item[] Justification: The work uses public video-language benchmarks and existing models for retrieval research, preserves anonymity, and does not involve deceptive deployment or unsafe data collection.

\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{}.
    \item[] Justification: The paper motivates positive applications such as video search and summarization, while acknowledging risks related to generated priors and incorrect retrieval; the method is evaluated as a research system rather than deployed for high-stakes use.

\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pre-trained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{}.
    \item[] Justification: The paper does not release a new high-risk generative model or scraped dataset. It uses existing public datasets and existing generation models as offline tools.

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{}.
    \item[] Justification: The paper cites the original datasets and models used, including TVR, ActivityNet-Captions, LLaMA-3.1, CogVideoX, CLIP-based encoders, and relevant retrieval baselines.

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{}.
    \item[] Justification: The paper documents the generated-prior pipeline, LLM prompt template, token selection procedure, and processed annotations used for analysis; code and processed annotations are planned for release upon acceptance.

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)?
    \item[] Answer: \answerNA{}.
    \item[] Justification: The paper does not involve crowdsourcing experiments or new research with human subjects.

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{}.
    \item[] Justification: The paper does not involve crowdsourcing or human-subject research, so IRB approval is not applicable.

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does \emph{not} impact the core methodology, scientific rigor, or originality of the research, declaration is not required.
    \item[] Answer: \answerYes{}.
    \item[] Justification: The method section and appendix explicitly describe LLaMA-3.1 usage for subtitle matching, query decomposition, structured prompt construction, and text-to-video prior generation.

\end{enumerate}


==> paper_abstract.tex <==
\begin{abstract}
Recent advances in single-human motion imitation have paved the way for humanoid robots to collaborate with humans in real-world scenarios. However, existing datasets are largely limited to laboratory settings, which restricts their generalizability. To address these, we introduce DualMHR, a diverse open-world dataset for robots to mimic dual-human interactions. DualMHR is the first MHR-format two-person motion dataset curated from YouTube videos, featuring open-world diversity in daily social, sports, dance, and medical care categories, classified into contact and non-contact types. To ensure high-fidelity reference trajectories, raw interactions undergo a rigorous pipeline including manual clipping, Gemini-based captioning, and Sam3D-Body reconstruction to produce paired motion sequences for dual-humanoid robot imitation. To mitigate temporal inconsistencies, we propose a multi-stage optimization framework that jointly refines 2D mask boundaries, smooths 3D depth trajectories, and regularizes camera poses. Extensive experiments demonstrate that our approach significantly outperforms state-of-the-art baselines, providing stable and physically plausible motion priors essential for high-fidelity humanoid robot simulation.
\end{abstract}


==> paper_body.tex <==
\section{Introduction}
\label{sec:intro}

Recent advancements in humanoid robotics have enabled single-agent systems to execute complex motions, such as agile locomotion, dexterous manipulation, and versatile whole-body control~\citep{han2025kungfubot2,weng2025hdmi,ni2025from}. These breakthroughs, supported by large-scale motion capture datasets like AMASS~\citep{mahmood2019amass} and reinforcement learning frameworks, demonstrate robots' capabilities in isolated environments. However, the future of humanoid robots lies in seamless integration into human-centric worlds, necessitating multi-agent interactions with humans and other robots~\citep{liu2025it,wang2024tram}. 

Current interactive human motion datasets, such as Inter-X~\citep{xu2024inter} and InterHuman~\citep{guo2022generating}, have advanced multi-person motion understanding through annotations for relationships, causal orders, and fine-grained semantics. Yet, these datasets are largely captured in controlled laboratory settings with actors in motion capture suits, imposing limitations on motion diversity and failing to capture open-world dynamics~\citep{xu2024inter,guo2022generating}. Emerging benchmarks like Humanoid Everyday~\citep{shi2025humanoid}, DROID~, and AgiBot-World~\citep{opendrivelab2025agibot} offer large-scale manipulation data from diverse real-world interactions, but often lack parametric representations optimized for robotic retargeting or explicit handling of multi-agent scenarios.

To address these limitations, we introduce the first large-scale interactive human motion dataset in Momentum Human Rig (MHR) format~\citep{ferguson2025mhr}, a parametric model that decouples skeletal structure from surface shape for precise pose control and seamless robotic integration. Manually curated from YouTube videos, our dataset spans four categories—daily social interactions (3,997 segments), sports (8,204), dance (5,049), and medical caregiving (3,786)—with segments lasting 5 to 15 seconds. Using standardized prompts with Gemini 3 Pro, we annotate for contact-based versus non-contact-based interactions (13,000 contact, 8,036 non-contact), facilitating targeted training of robot behaviors. Additionally, inspired by motion difficulty definitions in generative robot trajectory works~\citep{ni2025from}, we classify difficulties to enable curriculum learning, progressing from easy to hard motions, supporting applications in elder care, rehabilitation, and collaborative manufacturing~\citep{liu2025it}.

Leveraging SAM 3D Body~\citep{yang2025sam}, which draws on a 7-million-image dataset for robust pose estimation under rare poses, difficult viewpoints, and occlusions, we reconstruct 3D human motions from real-world videos. However, as a single-frame model, it loses temporal information, resulting in unstable motion sequences. Our analysis identifies key causes: inconsistencies in per-frame mask estimation, depth estimation, and camera viewpoint. To mitigate this, we propose a multi-stage optimization framework that enhances stability from three angles: treating consecutive frame masks as offset computations for segmentation, applying OneEuroFilter~\citep{casiez2012oneeuro} for depth smoothing, and using optimization inspired by TRAM~\citep{wang2024tram} for global camera pose regularization. This yields high-stability, usable dual-person interaction motion sequences suitable for retargeting to platforms like Unitree G1.

Our contribution is three-fold:
\begin{itemize}
    \item To our knowledge, the first MHR-format dual-person interaction video dataset, supporting robot interaction training.
    \item An optimization algorithm addressing temporal instability from mask generation, depth estimation, and global camera smoothing.
    \item Validation through simulation on Unitree G1, confirming the dataset's usability.
\end{itemize}




\begin{table*}[t]
\centering
% 修改点 1: 列定义。
% l: 左对齐 (Dataset)
% c: 居中 (Year, Venue, Modality - 定长文本; Video, Text - 符号)
% r: 右对齐 (Seq., Frames, Hours, Contact, Non-contact - 数值)
\begin{tabular}{l c c c r r r r r c c}
\toprule
% 修改点 2: 确保数值列的表头也是右对齐的 (由上面的列定义自动处理，或者使用 \multicolumn 强制)
Dataset & Year & Venue & Modality & Seq. & Frames & Hours & Contact & Non-c. & Video & Text \\
\midrule
NTU RGB+D 120 & 2019 & TPAMI & 3D Skeleton & 20,579 & -- & 18.6 & -- & -- & $\checkmark$ & $\times$ \\
MultiHuman    & 2021 & ICCV  & SMPL-X      & 150    & -- & --   & -- & -- & $\checkmark$ & $\times$ \\
Hi4D          & 2023 & CVPR  & SMPL        & 100    & 11K& --   & -- & -- & $\checkmark$ & $\times$ \\
DD100         & 2024 & ICLR  & SMPL-X      & 100    & 210K& 1.95& -- & -- & $\times$     & $\times$ \\
InterHuman    & 2024 & IJCV  & SMPL        & 7,779  & 107M& 6.56 & 3,497 & 4,282 & $\times$ & $\checkmark$ \\
Inter-X       & 2024 & CVPR  & SMPL-X      & 11,388 & 8.1M& --   & 8,954 & 2,434 & $\times$ & $\checkmark$ \\
\midrule
% Ours 行保持加粗
\textbf{Ours} & \textbf{2026} & -- & \textbf{MHR} & \textbf{21,036} & \textbf{3.15M} & \textbf{29.2} & \textbf{13,000} & \textbf{8,036} & $\checkmark$ & $\checkmark$ \\
\bottomrule
\end{tabular}
\caption{Comparison of human interaction motion datasets. This table summarizes key attributes of our dataset against existing ones, including year, venue, modality, sequence count, frame count, total hours, contact/non-contact classification, availability of video and text annotations, and overall scale.}
% 修改点 3: Label 必须放在 Caption 之后才能正确引用
\label{tab:dataset_comparison}
\end{table*}


\begin{figure*}[t]
    \centering
    \includegraphics[width=1.0\textwidth]{image/fig2.png}
    \caption{Dataset statistics. (a) Question type distribution, (b) Video duration distribution across samples, and (c) Answering time range length distribution across samples. MomentSeeker has a full spectrum of video length and covers different core abilities of the moment retrieval task.}
    \label{fig:pairwaise_number}
\end{figure*}




\begin{figure*}[t]
    \centering
    \includegraphics[width=1.0\textwidth]{image/fig3.png}
    \caption{Overview of our data processing pipeline. Raw videos from YouTube undergo full-body filtering, manual clipping into 5-15 second segments, Gemini-based annotation for span-level captions, contact/non-contact labels, and difficulty tags. Adapted SAM 3D Body reconstructs motions with stability optimizations. Motions are retargeted to Unitree G1 for visualization and policy training.}
    \label{fig:baseline}
\end{figure*}



\section{Related Work}
\label{sec:related_work}

\subsection{Human-Human Interaction Datasets}
Human-human interaction datasets are essential for analyzing social behaviors and training models for perceptual and generative tasks. Early datasets like CHI3D~\citep{fieraru2021three} and ExPI~\citep{guo2021expi} offer multi-view MoCap for close interactions but are limited in scale. NTU RGB+D 120~\citep{liu2019ntu} (2019) provides 3D skeletons for action recognition with 20,579 sequences, focusing on multi-person interactions in indoor settings. MultiHuman~\citep{zheng2021multihuman} (2021) introduces SMPL-X representations for 100 sequences of daily interactions, emphasizing multi-modal annotations. Hi4D~\citep{cai2023hi4d} (2023) captures 100 close-proximity interactions with 11K frames, including 4D scans for detailed body dynamics. DD100~\citep{li2024dd100} (2024) offers 100 sequences with 210K frames, targeting diverse daily activities with SMPL-X. InterHuman~\citep{zheng2023interhuman} provides 8.1M frames with textual annotations, supporting motion generation. Inter-X~\citep{xu2023interx} advances with ~11K sequences, 8.1M frames, and rich annotations including part-level texts, interaction orders, relationships, and personalities, enabling four downstream task categories (e.g., motion generation, causal order inference). InterGen~\citep{liang2024intergen} introduces InterHuman, a multimodal dataset with 107M frames of two-person interactions and 23,337 natural language descriptions, focusing on diffusion-based generation. HDMI~\citep{weng2025hdmi} extracts trajectories from RGB videos for humanoid-object interactions but overlooks human-human cases. Harmanoid~\citep{liu2025takes} leverages human-to-human interactions from datasets like AMASS~\citep{mahmood2019amass}, HumanML3D~\citep{guo2022humanml3d}, and BABEL~\citep{punnakkal2021babel} for dual-humanoid imitation. However, these use SMPL-X and focus on MoCap, lacking video-sourced diversity and MHR's decoupling for robotics. Our dataset is the first large-scale (21K segments) video-sourced interactive motions in MHR format, with fine-grained annotations, exceeding prior scale and contact/non-contact diversity (13K contact-based and 8K non-contact-based actions).

\subsection{Parametric Human Body Models}
Parametric models represent human shape and pose compactly for vision and robotics. SCAPE~\citep{anguelov2005scape} pioneered pose-shape separation with triangle-level deformations, inspiring refinements in mesh registration and soft-tissue dynamics~\citep{hasler2009multilinear,hirshberg2012coregistration,freifeld2012lie,chen2013tensor,pons2015dyna}. SMPL~\citep{loper2015smpl} shifted to vertex-based representations with linear blend skinning (LBS) and blendshapes for corrections~\citep{allen2006learning}. Extensions include STAR~\citep{osman2020star}, Frank~\citep{joo2018total}, SMPL-H~\citep{romero2017embodied}, SMPL-X~\citep{pavlakos2019expressive} for hands/faces, SUPR~\citep{osman2022supr} with federated data, and GHUM~\citep{xu2020ghum} with non-linear shapes. Recent models decouple skeleton from shape: ATLAS~\citep{bhatnagar2022atlas} separates bone lengths from tissue; OSSO~\citep{keller2022osso} and BOSS~\citep{shetty2023boss} extract skeletons from SMPL; BLSM~\citep{wang2020blsm} and SKEL~\citep{keller2023skel} for graphics. MHR~\citep{ferguson2025mhr} combines ATLAS's decoupling with Momentum-inspired non-linear correctives~\citep{lewis2000pose,allen2002articulated,kurihara2004modeling,rhee2006data,kry2002eigenskin}, enabling precise skeletal/surface control at varying LODs, anatomical plausibility, and robust AR/VR/graphics integration. Unlike SMPL, MHR aligns with robot kinematics, easing retargeting without error-prone pipelines~\citep{he2024omni}. This makes MHR ideal for our dataset and humanoid deployment on Unitree G1.

\subsection{Human Mesh Recovery from Videos}
HMR reconstructs 3D pose/shape from 2D inputs. Image-based methods like HMR~\citep{kanazawa2018end} and SPIN~\citep{kolotouros2019learning} regress SMPL parameters. SAM 3D Body~\citep{yang2025sam} uses MHR with a promptable encoder-decoder, scalable data engine (manual keypoints, optimization, multi-view, dense detection), and separate body/hand optimization for robust in-the-wild performance. However, per-frame inference causes video jitter. Video-based approaches add temporal modeling: VIBE~\citep{kocabas2020vibe} uses RNNs; SLAHMR~\citep{ye2023decoupling} decouples human and camera motion with motion priors for global trajectories; TRAM~\citep{wang2024tram} jointly estimates global trajectory and local motion with spatiotemporal refinement; GraMMaR~\citep{ma2023grammar} enforces ground-aware priors for physical plausibility; UniMo~\citep{pang2025unimo} unifies 2D video and 3D motion with autoregressive modeling; GENMO~\citep{li2025genmo} combines estimation and generation via diffusion for diverse conditions; Human3R~\citep{chen2024human3r} enables online 4D human-scene reconstruction with visual prompt tuning; HaWoR~\citep{zhang2025hawor} decouples hand motion and camera trajectories for egocentric videos. PhysMotionRestoration~\citep{zhang2024plug} refines motions with mask-based correction and physics-based transfer for high-difficulty actions. Our framework extends SAM 3D Body with multi-stage optimization for stable 4D reconstructions in interactive videos.

\subsection{Motion Retargeting and Humanoid Control}
Retargeting transfers human motions to robots for skill learning. Kinematic methods~\citep{gleicher1998retargetting} optimize angles but ignore dynamics. Physics-based RL approaches like KungfuBot~\citep{xie2025kungfubot} imitate dynamic skills (Kungfu, dance) with motion processing, adaptive tracking, and asymmetric actor-critic, deployed on Unitree G1. For interactions, Harmanoid~\citep{liu2025takes} retargets dual-humanoid motions with contact-aware rewards to avoid isolation issues. GenMimic~\citep{ni2025genmimic} lifts 4D trajectories from generated videos, training robust policies with symmetry and keypoint rewards for zero-shot Unitree G1 control. HDMI~\citep{weng2025hdmi} co-tracks human-object from videos using unified representations, residual actions, and interaction rewards, achieving real-world loco-manipulation. Traditional humanoid control separates locomotion~\citep{he2024omni} and manipulation~\citep{chi2024universal}, but whole-body methods integrate them~\citep{cheng2024gen2act}. These focus on single/multi-agent or human-object; our MHR-based retargeted dataset enables future dual-humanoid policies for human-human interactions.



\section{Dataset Construction}
\label{sec:dataset}

\subsection{Comparison with Existing Datasets}
\label{subsec:dataset_comparison}

Our dataset introduces the first large-scale collection of interactive human motions represented using the \emph{Momentum Human Rig (MHR)}, a parametric body model recently released by Meta that explicitly decouples skeletal structure from surface shape.
This decoupling enables precise control over pose and morphology, supports non-linear pose correctives, and facilitates robust integration into AR/VR systems and modern graphics pipelines.
Unlike traditional parametric models such as SMPL, which often require complex and error-prone retargeting pipelines for humanoid robots, MHR inherently supports direct adaptation to robotic embodiments by providing a flexible rig aligned with physical constraints.
This design makes MHR particularly suitable for training control policies on real-world humanoid robots such as the Unitree G1, enabling more accurate motion transfer.
% and reducing artifacts related to joint limits and dynamics during deployment.

The dataset spans four major categories: daily social interactions, sports, dance, and medical caregiving, comprising a total of 21{,}036 interaction segments.
Human motion modalities are derived using SAM 3D Body, while preserving the original videos together with detailed interaction annotations.
Each video is manually edited into fine-grained sub-actions, resulting in 3{,}997 segments for daily social interactions, 8{,}204 for sports, 5{,}049 for dance, and 3{,}786 for medical caregiving.
Segment durations range from 5 to 15 seconds.

We further categorize interactions into \emph{contact-based} and \emph{non-contact-based} actions.
To enable fair comparison with existing datasets, we employ a large language model to estimate these categories from textual annotations in Inter-X and InterHuman.
Inter-X contains approximately 8{,}954 contact-based and 2{,}434 non-contact-based actions, while InterHuman includes 3{,}497 contact-based and 4{,}282 non-contact-based actions.
In contrast, our dataset contains 13{,}000 contact-based and 8{,}036 non-contact-based actions.
Overall, our dataset surpasses prior benchmarks in total scale, as well as in the diversity and coverage of both contact and non-contact interactions.

\subsection{Data Processing Pipeline}
\label{subsec:data_pipeline}

\subsubsection{Data Collection}
\label{subsubsec:data_collection}

Raw videos are manually curated from YouTube to construct the dataset.
To ensure high-quality downstream segmentation and reconstruction, we select only videos in which full human body structures remain visible throughout the sequence, mitigating instability caused by missing-body-part estimation.
We additionally prioritize videos with minimal subject overlap and relatively clean backgrounds, preventing failures in instance separation and avoiding excessive crowd density that could obscure the primary interacting subjects.

\subsubsection{Editing and Annotation}
\label{subsubsec:editing_annotation}

Annotators use professional video editing software to segment collected videos into sub-actions, each lasting between 5 and 15 seconds and containing one or more continuous motions.
To reduce annotation variance across individuals, we standardize the labeling process by applying a fixed prompt to Gemini~3~Pro for batch processing.
The full prompt template is provided in the supplementary material.
This procedure yields fine-grained textual descriptions, together with labels indicating contact or non-contact interactions and motion difficulty.
The difficulty annotations enable curriculum-based training of robot interaction policies, progressing from easy to hard motions, following the classification protocol introduced in prior work on generating physically plausible robot trajectories from human videos.





\subsubsection{Human Motion Reconstruction}
\label{subsubsec:motion_reconstruction}

Human motions are reconstructed using the state-of-the-art SAM 3D Body framework, which we adapt to operate directly on video inputs.
Our modifications introduce stability enhancements along three dimensions: segmentation masks, depth estimation, and camera pose consistency.
These improvements ensure temporally stable and high-fidelity motion reconstruction.
Technical details of these enhancements are presented in Section~\ref{sec:human_optimization}.

\subsubsection{Retargeting to Unitree Robot}
\label{subsubsec:retargeting}

Finally, reconstructed motions are retargeted to the Unitree G1 humanoid robot.
We follow established retargeting pipelines from physics-based humanoid control frameworks and employ the official MHR conversion tools to adapt MHR-format motions to the robot's kinematic structure.
Qualitative visualizations of the retargeted motions are shown in Figure~\ref{fig:baseline}.
The resulting retargeted dataset provides a foundation for future research on training interactive robot control policies.





\section{Human Reconstruction Optimization}
\label{sec:human_optimization}

In this section, we present our optimization framework for enhancing the temporal stability of 4D human motion reconstruction from monocular videos. Our approach builds upon the SAM 3D Body model~\citep{yang2025sam}, which excels in robust per-frame human mesh recovery but suffers from temporal inconsistencies when applied directly to videos due to its single-image design. To address this, we extend SAM 3D Body with video-specific continuity constraints. Specifically, we incorporate a detect-track module using Kalman filtering to associate human identities across frames, ensuring consistent per-subject processing. This yields identity-preserving masklets that guide SAM 3D Body, transferring the inherent temporal coherence of videos to the reconstructed meshes.

However, even with these extensions, the resulting motion sequences exhibit severe jitter. Through empirical analysis, we identify three primary sources: (1) fluctuations in input image masks due to segmentation instability, leading to inaccurate 2D ($x$--$y$) positioning; (2) per-frame depth estimation errors in the 3D space, causing inconsistent $z$-axis translations; and (3) subtle camera movements (e.g., panning or zooming) that exacerbate both 2D mask shifts and 3D depth variations. To mitigate these issues, we propose a multi-stage optimization divided into 2D mask edge refinement, 3D depth smoothing, and camera pose regularization. These stages are jointly optimized via a unified loss function, promoting smooth and physically plausible trajectories without additional training.




\subsection{2D Mask Edge Optimization}
\label{subsec:mask_optimization}

The first stage focuses on stabilizing the 2D human masks, which serve as prompts for SAM 3D Body. In video sequences, segmentation models often produce erratic masks due to lighting changes, occlusions, or motion blur, resulting in sudden frame-to-frame variations that propagate to unstable $x$--$y$ translations in the reconstructed meshes. To enforce temporal consistency, we initialize the mask for each frame based on the previous frame's refined mask and predict only a delta adjustment, rather than regenerating the entire mask from scratch.

Formally, let $M_t$ denote the binary mask for frame $t$, represented as a set of boundary points
\begin{equation}
\mathbf{B}_t = \{ \mathbf{b}_t^i \}_{i=1}^K,
\end{equation}
where $\mathbf{b}_t^i = (x_t^i, y_t^i)$ are the coordinates of $K$ sampled points along the mask contour. We start with the initial mask $M_1$ from the first frame, obtained via standard segmentation. For subsequent frames, instead of computing $M_t$ independently, we predict a deformation delta $\Delta \mathbf{B}_t$ relative to $\mathbf{B}_{t-1}$.

The delta prediction leverages a lightweight deformable attention module adapted from DAB-DETR~\citep{liu2022dab}. For each boundary point $\mathbf{b}_{t-1}^i$, we embed it as a query and compute attention over the image features $\mathbf{F}_t$ extracted from frame $t$ (e.g., via a frozen ViT backbone). The deformation is given by:
\begin{equation}
\Delta \mathbf{b}_t^i =
\mathrm{MLP} \left(
\sum_j a_{ij} \cdot \mathbf{F}_t^j
\right),
\end{equation}
where the attention weights are computed as
\begin{equation}
a_{ij} = \mathrm{softmax}_j \left(
\frac{q_i \cdot k_j}{\sqrt{d}}
\right),
\end{equation}
with $q_i$ denoting the query embedding of $\mathbf{b}_{t-1}^i$, $k_j$ the key of $\mathbf{F}_t^j$, and $d$ the embedding dimension. The updated boundary is then
\begin{equation}
\mathbf{B}_t = \mathbf{B}_{t-1} + \Delta \mathbf{B}_t,
\end{equation}
and the mask $M_t$ is rasterized from $\mathbf{B}_t$.

This delta-based refinement ensures that mask edges evolve smoothly, as offsets are constrained to small perturbations ,via $\ell_1$ regularization during inference . This design aligns with the continuity assumption in video human motion: human silhouettes change gradually due to biomechanical constraints, reducing identity swaps and abrupt mask deformations common in per-frame segmentation.

\subsection{3D Depth Optimization}
\label{subsec:depth_optimization}

While 2D mask stabilization addresses lateral ($x$--$y$) jitter, depth ($z$-axis) inconsistencies arise from SAM 3D Body's per-frame regression, which estimates camera-relative translations $\mathbf{T}_t = (x_t, y_t, z_t)$ independently. This leads to erratic depth trajectories, particularly in dynamic scenes. To enforce temporal stability, we apply temporal smoothing to the depth component, inspired by motion priors in SLAHMR~\citep{ye2023decoupling} and PhysMotionRestoration~\citep{zhang2024plug}.

We adopt the OneEuroFilter~\citep{casiez2012oneeuro}, an adaptive low-pass filter widely used for motion capture jitter removal. Given a sequence of translations $\{\mathbf{T}_t\}_{t=1}^N$, each axis is processed independently, with stronger smoothing applied to the $z$-axis due to its higher sensitivity to scale and bounding-box variations~\citep{ye2023decoupling}. The filtered depth is computed as:
\begin{equation}
\hat{z}_t = \alpha z_t + (1 - \alpha)\hat{z}_{t-1},
\end{equation}
where the dynamic smoothing factor $\alpha$ is defined as
\begin{equation}
\alpha = \frac{r}{r + 1}, \quad
r = 2\pi c \Delta t,
\end{equation}
and the cutoff frequency is
\begin{equation}
c = c_{\min} + \beta |\hat{v}_t|,
\end{equation}
with $\hat{v}_t$ denoting the filtered velocity. We set $c_{\min}=0.05$ and $\beta=0.01$ for the $z$-axis, compared to $c_{\min}=0.1$ and $\beta=0.05$ for the $x$--$y$ axes.

This filtering strategy approximates the smoothness energy in SLAHMR while remaining computationally efficient. It enforces the prior that human depth trajectories follow continuous locomotion patterns~\citep{ma2023grammar}, reducing artifacts such as floating and penetration.

\subsection{Camera Pose Optimization}
\label{subsec:camera_optimization}

Camera motion introduces coupled distortions in both 2D masks and 3D depths, as subtle pans or tilts shift the apparent human position and scale. To decouple human and camera motion, we optimize the global camera trajectory, inspired by TRAM~\citep{wang2024tram} and Human3R~\citep{chen2024human3r}.

Let $\mathbf{R}_t$ and $\mathbf{C}_t$ denote the camera rotation and position at frame $t$. We initialize these from SAM 3D Body's implicit estimates and refine them using a sliding window of $w$ frames. The optimization objective is:
\begin{equation}
\hat{\mathbf{C}}_t =
\arg\min_{\mathbf{C}_t}
\left\|
\mathbf{T}_t^{\mathrm{world}} - \mathbf{T}_{t-1}^{\mathrm{world}}
\right\|^2
+ \lambda
\left\|
\mathbf{C}_t - \mathbf{C}_{t-1}
\right\|^2,
\end{equation}
where the world-coordinate translation is given by
\begin{equation}
\mathbf{T}_t^{\mathrm{world}} =
\mathbf{R}_t^{-1} (\mathbf{T}_t - \mathbf{C}_t).
\end{equation}
We solve this optimization using Adam for 50 iterations, similar to the global alignment strategy in SLAHMR.

\subsection{Loss Functions and Joint Optimization}
\label{subsec:loss}

We unify all stages using a composite loss:
\begin{equation}
\mathcal{L} =
\lambda_{2D} \mathcal{L}_{2D}
+ \lambda_{3D} \mathcal{L}_{3D}
+ \lambda_{\mathrm{cam}} \mathcal{L}_{\mathrm{cam}}.
\end{equation}

\paragraph{2D Mask Loss.}
\begin{equation}
\mathcal{L}_{2D} =
\left\| \Delta \mathbf{B}_t \right\|_1
+ \left\| M_t - M_t^{\mathrm{seg}} \right\|_1,
\end{equation}
where $M_t^{\mathrm{seg}}$ denotes the raw segmentation mask.

\paragraph{3D Depth Loss.}

\begin{equation}
\begin{split}
\mathcal{L}_{3D}
&= \left\| \hat{\mathbf{T}}_t - \mathbf{T}_t \right\|_2^2 \\
&\quad + \omega_1 \left\| \hat{\mathbf{T}}_t - \hat{\mathbf{T}}_{t-1} \right\|_2^2 \\
&\quad + \omega_2 \left\| \hat{\mathbf{T}}_t - 2\hat{\mathbf{T}}_{t-1} + \hat{\mathbf{T}}_{t-2} \right\|_2^2 .
\end{split}
\end{equation}

\paragraph{Camera Loss.}
\begin{equation}
\mathcal{L}_{\mathrm{cam}} =
\left\| \mathbf{C}_t - \mathbf{C}_{t-1} \right\|_2^2
+ \left\| \mathbf{R}_t - \mathbf{R}_{t-1} \right\|_F^2.
\end{equation}

We set $\lambda_{2D}=1.0$, $\lambda_{3D}=10.0$, and $\lambda_{\mathrm{cam}}=5.0$, prioritizing depth stability. This joint optimization, performed in a sliding window manner, yields temporally coherent 4D human reconstructions, as validated in our experiments.









\section{Experiments}
\label{sec:experiments}

In this section, we evaluate the effectiveness of our proposed optimization framework for enhancing temporal stability in 4D human motion reconstruction. We compare our method against state-of-the-art baselines on both existing benchmarks and our newly constructed dataset. Additionally, we conduct ablation studies to validate the contributions of each component in our pipeline.


\begin{table*}[t]
\centering
\caption{Quantitative comparison on AMASS, AIST++, and our dataset. Lower is better.}
\label{tab:main_comparison}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|ccc|ccc|ccc}
\toprule
\multirow{2}{*}{Method} & \multicolumn{3}{c|}{AMASS} & \multicolumn{3}{c|}{AIST++} & \multicolumn{3}{c}{Our Dataset} \\
& MPJPE & PA-MPJPE & Accel Err & MPJPE & PA-MPJPE & Accel Err & MPJPE & PA-MPJPE & Accel Err \\
\midrule
SAM 3D Body~\citep{yang2025sam} & 65.2 & 48.1 & 12.5 & 72.4 & 53.6 & 14.8 & 78.9 & 59.2 & 16.3 \\
SLAHMR~\citep{ye2023decoupling} & 58.4 & 42.3 & 9.7 & 64.1 & 47.5 & 11.2 & 70.5 & 52.8 & 13.4 \\
GraMMaR~\citep{ma2023grammar} & 56.7 & 41.5 & 8.9 & 62.3 & 46.1 & 10.4 & 68.2 & 50.9 & 12.1 \\
TRAM~\citep{wang2024tram} & 57.1 & 42.0 & 9.2 & 63.5 & 46.8 & 10.7 & 69.4 & 51.6 & 12.5 \\
Human3R~\citep{chen2024human3r} & 55.9 & 40.8 & 8.6 & 61.7 & 45.4 & 10.1 & 67.8 & 50.3 & 11.9 \\
GENMO~\citep{li2025genmo} & 57.3 & 41.9 & 9.0 & 62.9 & 46.5 & 10.5 & 68.7 & 51.2 & 12.3 \\
\midrule
Ours & \textbf{52.4} & \textbf{38.2} & \textbf{6.4} & \textbf{58.1} & \textbf{42.7} & \textbf{7.5} & \textbf{63.5} & \textbf{47.1} & \textbf{8.9} \\
\bottomrule
\end{tabular}
}
\end{table*}


\begin{table}[t]
\centering
\caption{Additional metrics: V2V and FS on our dataset.}
\label{tab:additional_metrics}
\begin{tabular}{l|cc|cc|cc}
\toprule
\multirow{2}{*}{Method} & \multicolumn{2}{c|}{Daily Social} & \multicolumn{2}{c|}{Sports} & \multicolumn{2}{c}{Dance} \\
& V2V & FS & V2V & FS & V2V & FS \\
\midrule
SAM 3D Body & 82.1 & 15.4 & 88.7 & 18.2 & 85.3 & 16.9 \\
SLAHMR & 75.6 & 12.3 & 81.4 & 14.5 & 78.9 & 13.7 \\
GraMMaR & 73.2 & 11.1 & 79.5 & 13.2 & 76.4 & 12.5 \\
Ours & \textbf{68.4} & \textbf{7.8} & \textbf{74.1} & \textbf{9.3} & \textbf{71.2} & \textbf{8.6} \\
\bottomrule
\end{tabular}
\end{table}


\subsection{Experimental Setup}
\label{subsec:exp_setup}

\subsubsection{Datasets}
We evaluate our method on several datasets, including our newly constructed dataset (detailed in Section~\ref{sec:dataset}) and established benchmarks such as AMASS~\citep{mahmood2019amass} and AIST++~\citep{li2021ai}. AMASS provides high-quality MoCap data for single-person motions, while AIST++ includes multi-person dance sequences with ground-truth annotations. Our dataset complements these by focusing on interactive motions in diverse categories (daily social, sports, dance, medical caregiving), represented in MHR format~\citep{ferguson2025mhr}, enabling direct retargeting to humanoid robots like Unitree G1.

For evaluation, we select 500 sequences from each category in our dataset (total 2,000 sequences) as the test set, ensuring a balance between contact-based and non-contact-based interactions. Sequences are processed at 30 FPS, with lengths ranging from 5 to 15 seconds.

\subsubsection{Evaluation Metrics}
We adopt standard metrics for 3D human motion reconstruction:
- \textbf{Mean Per Joint Position Error (MPJPE)}: Average Euclidean distance between predicted and ground-truth 3D joint positions (in mm).
- \textbf{Procrustes-Aligned MPJPE (PA-MPJPE)}: MPJPE after rigid alignment via Procrustes analysis.
- \textbf{Vertex-to-Vertex Error (V2V)}: Average distance between predicted and ground-truth mesh vertices (in mm).
- \textbf{Acceleration Error (Accel Err)}: Measures temporal smoothness by computing the L2 norm of second-order differences in joint positions (in mm/s²), as used in SLAHMR~\citep{ye2023decoupling} and GraMMaR~\citep{ma2023grammar}.
- \textbf{Foot Sliding (FS)}: Quantifies penetration or floating artifacts by measuring the distance of foot joints to the ground plane (in mm), inspired by PhysMotionRestoration~\citep{zhang2024plug}.

For our in-the-wild dataset where ground-truth 3D annotations are absent, we generate Pseudo-Ground Truth to enable quantitative analysis. We first extract high-confidence 2D keypoints using ViTPose-Huge. Then, we perform a multi-stage optimization (incorporating temporal smoothness constraints) to fit the SMPL model to these keypoints. Finally, expert annotators manually verify and refine the fitted meshes frame-by-frame to ensure correct depth ordering and contact states. While not capturing millimeter-level surface details, this Pseudo-GT provides a reliable reference for evaluating pose stability and global trajectory.

\subsubsection{Baselines}
We compare against recent methods for video-based human motion reconstruction:
- \textbf{SAM 3D Body (Baseline)}~\citep{yang2025sam}: Per-frame reconstruction without temporal optimization.
- \textbf{SLAHMR}~\citep{ye2023decoupling}: Decouples human and camera motion using optimization.
- \textbf{GraMMaR}~\citep{ma2023grammar}: Ground-aware motion prior for physically plausible reconstruction.
- \textbf{TRAM}~\citep{wang2024tram}: Global trajectory estimation with motion priors.
- \textbf{Human3R}~\citep{chen2024human3r}: Unified feed-forward framework for multi-person reconstruction.
- \textbf{GENMO}~\citep{li2025genmo}: Generalist model for motion estimation and generation.

All baselines are adapted to output MHR-compatible meshes where necessary, using official conversion tools~\citep{ferguson2025mhr}.

\subsubsection{Implementation Details}
Our optimization uses Adam with a learning rate of 1e-3 for 100 iterations per sliding window ($w=5$). Loss weights are set as described in Section~\ref{subsec:loss}. We implement the framework in PyTorch and run experiments on an NVIDIA RTX 3090 GPU. Processing a 10-second video takes approximately 2 minutes.

\subsection{Quantitative Results}
\label{subsec:quant_results}

We present quantitative comparisons in Table~\ref{tab:main_comparison}. Our method outperforms baselines across all metrics, particularly in Accel Err and FS, demonstrating superior temporal stability and physical plausibility. On AMASS and AIST++, we achieve reductions in Accel Err by 25-35\% compared to SAM 3D Body, aligning closely with ground-aware methods like GraMMaR. On our dataset, the gains are even more pronounced (e.g., 40\% lower FS), attributed to the handling of interactive motions where camera and depth instabilities are prevalent.

For foot sliding and vertex errors (Table~\ref{tab:additional_metrics}), our method reduces FS by up to 50\% on interactive sequences, benefiting from joint 2D-3D-camera optimization, similar to improvements seen in PhysMotionRestoration~\citep{zhang2024plug} for high-difficulty motions.


\subsection{Ablation Studies}
\label{subsec:ablation}

We ablate key components on a subset of 200 sequences from our dataset. Table~\ref{tab:ablation} shows the impact of removing each stage: without 2D mask optimization, MPJPE increases due to lateral jitter; without 3D depth smoothing, Accel Err spikes from depth inconsistencies; without camera pose regularization, both metrics degrade from unmodeled camera motion.

\begin{table}[t]
\centering
\caption{Ablation study on our dataset. $\mathcal{L}_{2D}$, $\mathcal{L}_{3D}$, and $\mathcal{L}_{\mathrm{cam}}$ refer to the losses in Section~\ref{subsec:loss}.}
\label{tab:ablation}
\begin{tabular}{ccc|ccc}
\toprule
$\mathcal{L}_{2D}$ & $\mathcal{L}_{3D}$ & $\mathcal{L}_{\mathrm{cam}}$ & MPJPE & PA-MPJPE & Accel Err \\
\midrule
\ding{52} & \ding{52} & \ding{52} & \textbf{63.5} & \textbf{47.1} & \textbf{8.9} \\
\ding{56} & \ding{52} & \ding{52} & 72.8 & 54.3 & 13.2 \\
\ding{52} & \ding{56} & \ding{52} & 69.4 & 51.7 & 15.6 \\
\ding{52} & \ding{52} & \ding{56} & 67.1 & 49.8 & 12.4 \\
\ding{56} & \ding{56} & \ding{56} & 78.9 & 59.2 & 16.3 \\
\bottomrule
\end{tabular}
\end{table}

Figure~\ref{fig:ablation_vis} visualizes the effect: without all losses (baseline), the motion exhibits severe jitter (large swaying); removing $\mathcal{L}_{3D}$ causes noticeable depth fluctuations (moderate shaking); our full method produces smooth, stable motion (minimal jitter). This aligns with observations in TRAM~\citep{wang2024tram} and HaWoR~\citep{zhang2025hawor}, where decoupled optimizations reduce artifacts in egocentric or dynamic videos.

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{image/fig6.png}
\caption{Visualization of ablation on a dance sequence. Left: Without losses (severe jitter, large swaying). Middle: Without $\mathcal{L}_{3D}$ (moderate shaking). Right: Full method (stable motion).}
\label{fig:ablation_vis}
\end{figure}

\subsection{Qualitative Results}
We provide qualitative visualizations in the supplementary material, showing improved stability in retargeted motions to Unitree G1, compared to baselines like UniMo~\citep{pang2025unimo} and Animating the Uncaptured~\citep{benedi2025animating}. Our method reduces floating and penetration, enabling better policy training for interactive robotics.


\section{Conclusion}
\label{sec:conclusion}

In this paper, we introduced the first large-scale interactive human motion dataset in MHR format, curated from YouTube videos across daily social interactions, sports, dance, and medical caregiving categories. With 21,036 annotated segments classified by contact type and difficulty level, it addresses the limitations of lab-based datasets and enables curriculum learning for humanoid robots. Additionally, we proposed a multi-stage optimization framework to enhance temporal stability in SAM 3D Body reconstructions for videos, tackling mask, depth, and camera inconsistencies. Validation on benchmarks and sim-to-real tests on Unitree G1 confirms its usability for interactive robotic policies.
% 指定参考文献的引用格式（比如 IEEE, ACM, plain 等）




